Unsupervised Novel View Synthesis from a Single Image

Novel view synthesis from a single image has recently achieved remarkable results, although the requirement of some form of 3D, pose, or multi-view supervision at training time limits the deployment in real scenarios. This work aims at relaxing these assumptions enabling training of conditional generative models for novel view synthesis in a completely unsupervised manner. We first pre-train a purely generative decoder model using a 3D-aware GAN formulation while at the same time train an encoder network to invert the mapping from latent space to images. Then, we swap encoder and decoder and train the network as a conditioned GAN with a mixture of an autoencoder-like objective and self-distillation. At test time, given a view of an object, our model first embeds the image content in a latent code and regresses its pose, then generates novel views of it by keeping the code fixed and varying the pose. We test our framework on both synthetic datasets such as ShapeNet and on unconstrained collections of natural images, where no competing methods can be trained.

==> graf.tex <==
\section{Preliminary Results with a Different Decoder}
\label{sec:graf}

We report preliminary results obtained changing the decoder network in our formulation with the recently proposed neural radiance field based GRAF \cite{schwarz2020graf}.
While the architecture of the network is quite different from the HoloGAN \cite{Nguyen-Phuoc_2019_ICCV} one used throughout the paper, from a black box perspective, both models allow to provide a latent vector and a pose to generate a view of an object and can therefore be in principle interchanged in our framework.

While the swap does not require major changes, the computational cost of rendering a full image using GRAF is significantly higher.
Thus, following the same strategy as its authors, we train on patches.
However, the encoder requires an entire image to estimate $z$ and $\theta$. Thus, in stage 1, we initialize GRAF with the pretrained weights released by the authors, and we train only the encoder $E$ to invert images to the generator latent space.
Then, in stage 2 due to the patch generation we did not use $L_{VGG}$ and $L_{SSIM}$ to measure the reconstruction error, but we rely only on the pixel-wise $L_2$ loss. 

%\footnote{\href{https://github.com/autonomousvision/graf/blob/main/configs/pretrained\_models.yaml}{https://github.com/autonomousvision/graf/blob/main/configs/pretrained\_models.yaml}}. 

In \cref{fig:graf_multiple_stages}, we report results obtained from a Stage 1, Stage 2 and a Fine-tuned network on the Carla dataset \cite{schwarz2020graf}. As we can see from the picture, Stage 1  is not sufficient to obtain a good reconstruction, while we can recover the identity of the input car in Stage 2. Then, during the Fine-tuning we recover some details of the input image such as the color and the pose. In \cref{fig:graf_rotations} we report some qualitative results of generated novel views for the same input images showing how the multi-view consistency of the models is maintained.

\begin{figure}
    \newlength{\grafmultiplestagesWidth}
    \setlength{\grafmultiplestagesWidth}{0.18\linewidth}
    \centering
    \begin{tabular}{c|ccc}
        \toprule
        Input & Stage 1 & Stage 2 & Finetune \\
        \midrule
        \includegraphics[width=\grafmultiplestagesWidth]{images/graf/008000/input.png} &
        \includegraphics[width=\grafmultiplestagesWidth]{images/graf/008000/stage1/predicted.png} &
        \includegraphics[width=\grafmultiplestagesWidth]{images/graf/008000/stage2/predicted.png} &
        \includegraphics[width=\grafmultiplestagesWidth]{images/graf/008000/stage3/predicted.png} \\
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008001/input.png} &
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008001/stage1/predicted.png} &
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008001/stage2/predicted.png} &
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008001/stage3/predicted.png} \\
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008002/input.png} &
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008002/stage1/predicted.png} &
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008002/stage2/predicted.png} &
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008002/stage3/predicted.png} \\
        
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008003/input.png} &
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008003/stage1/predicted.png} &
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008003/stage2/predicted.png} &
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008003/stage3/predicted.png} \\
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008004/input.png} &
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008004/stage1/predicted.png} &
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008004/stage2/predicted.png} &
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008004/stage3/predicted.png} \\
        \includegraphics[width=\grafmultiplestagesWidth]{images/graf/008005/input.png} &
        \includegraphics[width=\grafmultiplestagesWidth]{images/graf/008005/stage1/predicted.png} &
        \includegraphics[width=\grafmultiplestagesWidth]{images/graf/008005/stage2/predicted.png} &
        \includegraphics[width=\grafmultiplestagesWidth]{images/graf/008005/stage3/predicted.png} \\
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008006/input.png} &
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008006/stage1/predicted.png} &
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008006/stage2/predicted.png} &
        %\includegraphics[width=\grafmultiplestagesWidth]{images/graf/008006/stage3/predicted.png} \\
        \includegraphics[width=\grafmultiplestagesWidth]{images/graf/008007/input.png} &
        \includegraphics[width=\grafmultiplestagesWidth]{images/graf/008007/stage1/predicted.png} &
        \includegraphics[width=\grafmultiplestagesWidth]{images/graf/008007/stage2/predicted.png} &
        \includegraphics[width=\grafmultiplestagesWidth]{images/graf/008007/stage3/predicted.png} \\
    \bottomrule
    \end{tabular}
    \caption{Qualitative comparison of a Stage 1, Stage 2 and Fine-Tuning network using as decoder GRAF \cite{schwarz2020graf} instead of HoloGAN \cite{Nguyen-Phuoc_2019_ICCV} on the Carla dataset.}
    \label{fig:graf_multiple_stages}
\end{figure}


\begin{figure*}
    \newlength{\grafRotationWidth}
    \setlength{\grafRotationWidth}{0.12\linewidth}
    \centering
    \begin{tabular}{c|ccccc}
        \toprule
        Input & \multicolumn{5}{c}{$\theta$ Interpolation}\\
        \midrule
        \includegraphics[width=\grafRotationWidth]{images/graf/008000/input.png} &
        \includegraphics[width=\grafRotationWidth]{images/graf/008000/stage3/rgb_0000.png} &
        \includegraphics[width=\grafRotationWidth]{images/graf/008000/stage3/rgb_0005.png} &
        \includegraphics[width=\grafRotationWidth]{images/graf/008000/stage3/rgb_0010.png} &
        \includegraphics[width=\grafRotationWidth]{images/graf/008000/stage3/rgb_0015.png} &
        \includegraphics[width=\grafRotationWidth]{images/graf/008000/stage3/rgb_0019.png} \\
        
        % \includegraphics[width=\grafRotationWidth]{images/graf/008000/input.png} &
        % \includegraphics[width=\grafRotationWidth]{images/graf/008000/stage3/depth_0000.png} &
        % \includegraphics[width=\grafRotationWidth]{images/graf/008000/stage3/depth_0005.png} &
        % \includegraphics[width=\grafRotationWidth]{images/graf/008000/stage3/depth_0010.png} &
        % \includegraphics[width=\grafRotationWidth]{images/graf/008000/stage3/depth_0015.png} &
        % \includegraphics[width=\grafRotationWidth]{images/graf/008000/stage3/depth_0019.png} \\
        
        %\includegraphics[width=\grafRotationWidth]{images/graf/008001/input.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008001/stage3/rgb_0000.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008001/stage3/rgb_0005.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008001/stage3/rgb_0010.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008001/stage3/rgb_0015.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008001/stage3/rgb_0019.png} \\
        
        %\includegraphics[width=\grafRotationWidth]{images/graf/008002/input.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008002/stage3/rgb_0000.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008002/stage3/rgb_0005.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008002/stage3/rgb_0010.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008002/stage3/rgb_0015.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008002/stage3/rgb_0019.png} \\
        
        %\includegraphics[width=\grafRotationWidth]{images/graf/008003/input.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008003/stage3/rgb_0000.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008003/stage3/rgb_0005.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008003/stage3/rgb_0010.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008003/stage3/rgb_0015.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008003/stage3/rgb_0019.png} \\
        
        %\includegraphics[width=\grafRotationWidth]{images/graf/008004/input.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008004/stage3/rgb_0000.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008004/stage3/rgb_0005.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008004/stage3/rgb_0010.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008004/stage3/rgb_0015.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008004/stage3/rgb_0019.png} \\
        
        \includegraphics[width=\grafRotationWidth]{images/graf/008005/input.png} &
        \includegraphics[width=\grafRotationWidth]{images/graf/008005/stage3/rgb_0000.png} &
        \includegraphics[width=\grafRotationWidth]{images/graf/008005/stage3/rgb_0005.png} &
        \includegraphics[width=\grafRotationWidth]{images/graf/008005/stage3/rgb_0010.png} &
        \includegraphics[width=\grafRotationWidth]{images/graf/008005/stage3/rgb_0015.png} &
        \includegraphics[width=\grafRotationWidth]{images/graf/008005/stage3/rgb_0019.png} \\
        
        % \includegraphics[width=\grafRotationWidth]{images/graf/008005/input.png} &
        % \includegraphics[width=\grafRotationWidth]{images/graf/008005/stage3/depth_0000.png} &
        % \includegraphics[width=\grafRotationWidth]{images/graf/008005/stage3/depth_0005.png} &
        % \includegraphics[width=\grafRotationWidth]{images/graf/008005/stage3/depth_0010.png} &
        % \includegraphics[width=\grafRotationWidth]{images/graf/008005/stage3/depth_0015.png} &
        % \includegraphics[width=\grafRotationWidth]{images/graf/008005/stage3/depth_0019.png} \\
        
        %\includegraphics[width=\grafRotationWidth]{images/graf/008006/input.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008006/stage3/rgb_0000.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008006/stage3/rgb_0005.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008006/stage3/rgb_0010.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008006/stage3/rgb_0015.png} &
        %\includegraphics[width=\grafRotationWidth]{images/graf/008006/stage3/rgb_0019.png} \\
        
        \includegraphics[width=\grafRotationWidth]{images/graf/008007/input.png} &
        \includegraphics[width=\grafRotationWidth]{images/graf/008007/stage3/rgb_0000.png} &
        \includegraphics[width=\grafRotationWidth]{images/graf/008007/stage3/rgb_0005.png} &
        \includegraphics[width=\grafRotationWidth]{images/graf/008007/stage3/rgb_0010.png} &
        \includegraphics[width=\grafRotationWidth]{images/graf/008007/stage3/rgb_0015.png} &
        \includegraphics[width=\grafRotationWidth]{images/graf/008007/stage3/rgb_0019.png}\\
        \bottomrule
    \end{tabular}
    \caption{Novel view synthesis from a single input image using as our decoder GRAF \cite{schwarz2020graf} instead of HoloGAN \cite{Nguyen-Phuoc_2019_ICCV} on the Carla dataset.}
    \label{fig:graf_rotations}
\end{figure*}


==> images/ablation/ablation.tex <==
\begin{figure}
	\setlength{\tabcolsep}{1pt}
	\centering
	\begin{tabular}{ccccccc}
	Input & Rec. & 36$^{\circ}$ & 108$^{\circ}$ & 288$^{\circ}$ \\
	\includegraphics[width=0.09\textwidth]{images/ablation/286_inputs_0.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625311/286_samples_0_0.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625311/286_samples_0_2.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625311/286_samples_0_6.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625311/286_samples_0_16.png} \\
    & 
	\includegraphics[width=0.09\textwidth]{images/ablation/18625022/286_samples_0_0.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625022/286_samples_0_2.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625022/286_samples_0_6.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625022/286_samples_0_16.png} \\
	 &
	\includegraphics[width=0.09\textwidth]{images/ablation/no_multiview/286_samples_0_0.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/no_multiview/286_samples_0_2.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/no_multiview/286_samples_0_6.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/no_multiview/286_samples_0_16.png} \\
	 &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625024/286_samples_0_0.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625024/286_samples_0_2.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625024/286_samples_0_6.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625024/286_samples_0_16.png} \\
	 &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625026/286_samples_0_0.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625026/286_samples_0_2.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625026/286_samples_0_6.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625026/286_samples_0_16.png} \\
	 &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625367/286_samples_0_0.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625367/286_samples_0_2.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625367/286_samples_0_6.png} &
	\includegraphics[width=0.09\textwidth]{images/ablation/18625367/286_samples_0_16.png} \\
	\end{tabular}
	\caption{Ablation qualitative results. Rows from 1 to 5: only stage 2, + stage 1, + self-distillation, + multi-view on generated, + adversarial, + cycle losses on generated.}
	\label{fig:ablation_qualitatives}
\end{figure}

==> images/finetune.tex <==
\begin{figure*}
	\setlength{\tabcolsep}{1pt}
	\centering
	\setlength{\fboxrule}{2pt} 
	\setlength{\fboxsep}{0pt} 
	\scalebox{0.9}{
	\begin{tabular}{ccccccc}
	Input. & \multicolumn{6}{c}{$\theta$ Interpolation} \\
	\fbox{\includegraphics[width=0.13\textwidth]{images/finetuning/191257.png}} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/191257/0_samples_0_2.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/191257/0_samples_0_5.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/191257/0_samples_0_8.png} &
	\fbox{\includegraphics[width=0.13\textwidth]{images/finetuning/191257/reconstruction_191257.png}} &
	%\includegraphics[width=0.13\textwidth]{images/finetuning/191257/0_samples_0_11.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/191257/0_samples_0_14.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/191257/0_samples_0_17.png} \\
	&
	\includegraphics[width=0.13\textwidth]{images/finetuning/191257_finetuning/0_samples_0_2.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/191257_finetuning/0_samples_0_5.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/191257_finetuning/0_samples_0_8.png} &
    \fbox{\includegraphics[width=0.13\textwidth]{images/finetuning/191257_finetuning/rec.png}} &
	%\includegraphics[width=0.13\textwidth]{images/finetuning/191257_finetuning/0_samples_0_11.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/191257_finetuning/0_samples_0_14.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/191257_finetuning/0_samples_0_17.png} \\
	\fbox{\includegraphics[width=0.13\textwidth]{images/finetuning/d1bd31d2a90375.jpg}} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/d1bd31d2a90375/0_samples_0_8.png} &
	%\includegraphics[width=0.13\textwidth]{images/finetuning/d1bd31d2a90375/0_samples_0_17.png} &
	\fbox{\includegraphics[width=0.13\textwidth]{images/finetuning/d1bd31d2a90375/reconstruction_d1bd31d2a90375.jpg}} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/d1bd31d2a90375/0_samples_0_23.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/d1bd31d2a90375/0_samples_0_29.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/d1bd31d2a90375/0_samples_0_35.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/d1bd31d2a90375/0_samples_0_4.png} \\
	&
	\includegraphics[width=0.13\textwidth]{images/finetuning/d1bd31d2a90375_finetuning/0_samples_0_8.png} &
	%\includegraphics[width=0.13\textwidth]{images/finetuning/d1bd31d2a90375_finetuning/0_samples_0_17.png} &
	\fbox{\includegraphics[width=0.13\textwidth]{images/finetuning/d1bd31d2a90375_finetuning/rec.png}} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/d1bd31d2a90375_finetuning/0_samples_0_23.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/d1bd31d2a90375_finetuning/0_samples_0_29.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/d1bd31d2a90375_finetuning/0_samples_0_35.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/d1bd31d2a90375_finetuning/0_samples_0_4.png} \\
	
	\end{tabular}}
	\caption{Qualitative comparison between results of stage 2 (first and third rows) and fine-tuning (second and fourth rows) on CelebA and Real Cars datasets. Reconstructed images with predicted pose are framed.}
	\label{fig:finetune}
\end{figure*}


\iffalse
\begin{figure*}
	\setlength{\tabcolsep}{1pt}
	\centering
	\begin{tabular}{cccccccccc}
	Input & -40$^{\circ}$ & -30$^{\circ}$ & -20$^{\circ}$ & -10$^{\circ}$ & 0$^{\circ}$ & 10$^{\circ}$ & 20$^{\circ}$ & 30$^{\circ}$ & 40$^{\circ}$ \\
	\includegraphics[width=0.13\textwidth]{images/finetuning/3_inputs_0.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/3_samples_0_1.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/3_samples_0_2.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/3_samples_0_3.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/3_samples_0_4.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/3_samples_0_5.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/3_samples_0_6.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/3_samples_0_7.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/3_samples_0_8.png} &
	\includegraphics[width=0.13\textwidth]{images/finetuning/3_samples_0_9.png} \\
	\end{tabular}
	\caption{Qualitative results for celebA - Finetuning.}
	\label{fig:swap_pose_celebA}
\end{figure*}
\fi

==> images/fitting.tex <==
	\begin{figure}
		\setlength{\tabcolsep}{1pt}
		\centering
    	\setlength{\fboxrule}{2pt} 
    	\setlength{\fboxsep}{0pt}
    	\scalebox{0.75}{
		\begin{tabular}{ccccc}
			\tabcolsep0em
			& Input & -25$^{\circ}$ & Rec. & 25$^{\circ}$ \\
			
	        \rotatebox{90}{\hspace{0.6cm} \cite{creswellTNNL2019}} &
			\fbox{\includegraphics[width=0.11\textwidth]{images/fitting/190415.png}} &
			\includegraphics[width=0.11\textwidth]{images/fitting/fit_nostage1_0_samples_0_5.png} &
			\fbox{\includegraphics[width=0.11\textwidth]{images/fitting/fit_nostage1_0_samples_0_10.png}} &
			\includegraphics[width=0.11\textwidth]{images/fitting/fit_nostage1_0_samples_0_15.png} \\
		    \rotatebox{90}{\hspace{0.6cm} \cite{zhuECCV2016}} &
			\fbox{\includegraphics[width=0.11\textwidth]{images/fitting/190415.png}} &
			\includegraphics[width=0.11\textwidth]{images/fitting/fit_0_samples_0_5.png} &
			\fbox{\includegraphics[width=0.11\textwidth]{images/fitting/fit_0_samples_0_10.png}} &
			\includegraphics[width=0.11\textwidth]{images/fitting/fit_0_samples_0_15.png} \\
			\rotatebox{90}{\hspace{0.4cm} Stage2} &
		    \fbox{\includegraphics[width=0.11\textwidth]{images/fitting/190415.png}} &
			\includegraphics[width=0.11\textwidth]{images/fitting/stage2_0_samples_0_5.png} &
			\fbox{\includegraphics[width=0.11\textwidth]{images/fitting/stage2_0_samples_0_10.png}} &
			\includegraphics[width=0.11\textwidth]{images/fitting/stage2_0_samples_0_15.png} \\
		    \rotatebox{90}{\hspace{0.1cm} Stage2+Ft.} &
			\fbox{\includegraphics[width=0.11\textwidth]{images/fitting/190415.png}} &
			\includegraphics[width=0.11\textwidth]{images/fitting/0_samples_0_5.png} &
			\fbox{\includegraphics[width=0.11\textwidth]{images/fitting/0_samples_0_10.png}} &
			\includegraphics[width=0.11\textwidth]{images/fitting/0_samples_0_15.png} \\	
		\end{tabular}}
		\caption{Qualitative comparison between different inversion strategies.
		From top to bottom: \cite{creswellTNNL2019}, \cite{zhuECCV2016}, our Stage 2, our Stage2 + image-specific finetuning. From left to right: input, azimuth rotations respect to the input of -25$^{\circ}$, 0$^{\circ}$(reconstruction), and 25$^{\circ}$.}
		\label{fig:fitting}
	\end{figure}

==> images/swap_poses.tex <==
	\begin{figure}
		\setlength{\tabcolsep}{1pt}
		\centering
		\begin{tabular}{ccccc}
			\tabcolsep 0em
			\diagbox[height=1.25\rotheadsize]{\raisebox{3ex}{$z$}}{\raisebox{-4ex}{Pose}} &
			\includegraphics[width=0.09\textwidth]{images/swap_poses/references/182662.png} &
			\includegraphics[width=0.09\textwidth]{images/swap_poses/references/182769.png} &
			\includegraphics[width=0.09\textwidth]{images/swap_poses/references/182929.png} &
			\includegraphics[width=0.09\textwidth]{images/swap_poses/references/182994.png}
			%\includegraphics[width=0.09\textwidth]{images/swap_poses/references/185368.png} 
			\\
			\includegraphics[width=0.09\textwidth]{images/swap_poses/182641/182641.png} &
			%\includegraphics[width=0.09\textwidth]{images/swap_poses/182641/182641_reconstructed.png} &
			\includegraphics[width=0.09\textwidth]{images/swap_poses/182641/182662_reposed.png} &
			\includegraphics[width=0.09\textwidth]{images/swap_poses/182641/182769_reposed.png} &
			\includegraphics[width=0.09\textwidth]{images/swap_poses/182641/182929_reposed.png} &
			\includegraphics[width=0.09\textwidth]{images/swap_poses/182641/182994_reposed.png}
			%\includegraphics[width=0.09\textwidth]{images/swap_poses/182641/185368_reposed.png}
			\\
			\includegraphics[width=0.09\textwidth]{images/swap_poses/182659/182659.png} &
			%\includegraphics[width=0.09\textwidth]{images/swap_poses/182659/reconstructed_182659.png} &
			\includegraphics[width=0.09\textwidth]{images/swap_poses/182659/182662_reposed.png} &
			\includegraphics[width=0.09\textwidth]{images/swap_poses/182659/182769_reposed.png} &
			\includegraphics[width=0.09\textwidth]{images/swap_poses/182659/182929_reposed.png} &
			\includegraphics[width=0.09\textwidth]{images/swap_poses/182659/182994_reposed.png}
			%\includegraphics[width=0.09\textwidth]{images/swap_poses/182659/185368_reposed.png}
			\\
		\end{tabular}
		\caption{Qualitative pose estimation results on CelebA. We extract $\theta$ from $I_{\theta}$ images (first row) and $z$ from $I_z$ images (first column) to craft a novel image.}
		\label{fig:swap_pose_celebA}
	\end{figure}
